Optimistic Rates for Learning from Label Proportions

We consider a weakly supervised learning problem called Learning from Label Proportions (LLP), where examples are grouped into ``bags'' and only the average label within each bag is revealed to the learner. We study various learning rules for LLP that achieve PAC learning guarantees for classification loss. We establish that the classical Empirical Proportional Risk Minimization (EPRM) learning rule (Yu et al., 2014) achieves fast rates under realizability, but EPRM and similar proportion matching learning rules can fail in the agnostic setting. We also show that (1) a debiased proportional square loss, as well as (2) a recently proposed EasyLLP learning rule (Busa-Fekete et al., 2023) both achieve ``optimistic rates'' (Panchenko, 2002); in both the realizable and agnostic settings, their sample complexity is optimal (up to log factors) in terms of $\epsilon, \delta$, and VC dimension.

==> empirical_results.tex <==
\section{Experiments on MNIST}

\begin{itemize}
    \item Synthetic experiment on 1D prediction for linear thresholds, demonstrating that the two-step estimator closely matches the performance of the best estimator in all regimes $\eta \in [0,1/2]$.
    \item Experiments on MNIST Odd vs Even. Main takeaways:
    \begin{itemize}
        \item Performance for Adam and SGD can be different, as well as with different learning rates.
        \item Biased Square Loss seems to work best, with less overfitting than the other loss functions. For Adam, the aggregate log loss also does well, but not with SGD.
    \end{itemize}
    \item \GLcomment{Further experiments: MNIST 1 vs All, CIFAR 10, Criteo?}
\end{itemize}


\subsection{Bag Size 10}
\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-adam-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using Adam for Bag Size 10, Various Learning Rates}
\end{figure}

\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag10/bag10-sgd-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using SGD for Bag Size 10, Various Learning Rates}
\end{figure}


\subsection{Bag Size 100}
\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-adam-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using Adam for Bag Size 10, Various Learning Rates}
\end{figure}

\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag100/bag100-sgd-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using SGD for Bag Size 100, Various Learning Rates}
\end{figure}



\subsection{Bag Size 1000}
\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-adam-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using Adam for Bag Size 10, Various Learning Rates}
\end{figure}

\begin{figure}[H]
	\centering
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.05.png}
		\caption{LR $=.05$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.01.png}
		\caption{LR $=.01$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.005.png}
		\caption{LR $=.005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.001.png}
		\caption{LR $=.001$}
	\end{subfigure}
 \vspace{0cm}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.0005.png}
		\caption{LR $=.0005$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr0.0001.png}
		\caption{LR $=.0001$}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr5e-05.png}
		\caption{LR $=.00005$}
	\end{subfigure}
 \begin{subfigure}{.24\textwidth}
		\includegraphics[width=\textwidth]{figures/bag1000/bag1000-sgd-lr1e-05.png}
		\caption{LR $=.00001$}
	\end{subfigure}
 \caption{MNIST Odd vs Even using SGD for Bag Size 1000, Various Learning Rates}
\end{figure}

==> older_notes.tex <==
\section{Notes for the Arxiv version}
\begin{enumerate}
    \item We can prove optimistic rates for a broad class of estimators which generalize EasyLLP, and can be viewed as different "proportion matching" losses. This can be done with the offset method. Have some theorem to this effect which generalizes the EasyLLP result.
    \item Illustration of different variance properties using simulation.
    \item The debiased square loss we consider in the paper is basically a variance reduced version of the square loss estimator from above. In addition to having the optimistic rate for learning we also have the optimistic rate for estimation (i.e., a localized uniform convergence bound).
    \item What happens if we try to apply these learning rules to gradient based learning. Experimental evidence suggests that there is some benefit to the previous point, that the debiased square loss does better than other estimates.
    \item One experiment to try is to plot some measure of the variance of the loss estimate throughout training (on both the training and test set). I would expect the variance for the debiased square loss to reduce throughout training, but not so for EasyLLP.
    \item other experiments: 1 vs All MNIST, CIFAR 10 1 vs All and Animal vs machine, see EasyLLP paper for their experiments.
\end{enumerate}

% \section{Related Works}
% \begin{itemize}
%     \item EasyLLP \cite{busa2023easy}: a general surrogate label approach.
%     \item \cite{yu2014learning}: first prove generalization guarantee for learning the bag proportions then show how to get upper bounds on the individual label errors.
%     \item SVM approaches: \cite{yu2013proptosvm, qi2016learning, shi2019learning}
%     \item Curated vs Random Bags \cite{chen2023learning}: shows how curated bags where the bags are sorted according to the features can improve the sample complexity. For random bags using a corrected $\ell_2$ loss they give a generalization bound.
%     \item Papers by Saket on computing LTFs from LLP data: \cite{saket2021learnability, saket2022algorithms}
%     \item Combining bags may help: \cite{saket2022combining}
%     \item MeanMap \cite{quadrianto2008estimating}: models the problem as exponential family.
%     \item Deep multi-class learning \cite{dulac2019deep}: A label generation approach that can work for DNNs!
%     \item Papers by Clayton Scott: \cite{scott2020learning, zhang2022learning}. The first one has an interesting counterexample for EPR. Second one is a multi-class extension to the first.
% \end{itemize}

\section{Practical Learning Rules: Minimizing Surrogate Losses}
In this section, we investigate whether a similar equivalence holds for surrogate loss functions. \GLcomment{not really sure if we can say anything interesting theoretically, but experimental comparisons are nice.}

\subsection{Square Loss}
We have the following proposition.
\begin{proposition}\label{prop:equiv-sq}
Consider the loss function $\ell(f,(x,y)) = \prn{f(x) - y}^2$. Define the respective square and reverse square losses as
\begin{align*}
    \lossbagsq(f, B) &\coloneqq k \cdot \prn*{ \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 - \frac{1}{k} \sum_{i \ne j} (f(x_i) - p) (f(x_j) - p)\\
    \lossbagrsq(f, B) &\coloneqq 1 - k \cdot \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 + \frac{1}{k} \cdot \prn*{\sum_{i\ne j} (f(x_i) + p - 1)(f(x_j) + p - 1)} \\
    &\quad\quad\quad + \frac{2}{k} \prn*{\sum_i f(x_i)^2 - f(x_i)}.
\end{align*}
Then for any predictor $f$ and bag $B$ we have
\begin{align*}
    \losseasysq(f, B) = \frac{1}{2} \prn*{\lossbagsq(f, B) + \lossbagrsq(f, B)}.
\end{align*}
\end{proposition}
Note that there is an additional correction term $\frac{2}{k} \prn*{\sum_i f(x_i)^2 - f(x_i)}$, which is needed for the equivalence to hold. The proof for \pref{prop:equiv-sq} is similar to that of \pref{prop:easyLLP-equivalence}.

With the square loss, we naturally have an algorithmic approach to solve classifcation in aggregate learning. Let $\cF_\Theta = \crl{f_\theta: \theta \in \Theta}$ be a continuously parameterized function class. Consider the loss function:
$\ell_\gamma(f_\theta, B) = (1-\gamma) \ell_\mathrm{sq}(f_\theta, B) + \gamma \ell_\mathrm{rsq}(f_\theta, B)$. EasyLLP corresponds to picking $\gamma = 1/2$. However, we can pick other choices of $\gamma$. Our intuition says that $\gamma$ should be small if we are realizable, since the variance of this estimate is reduced. The loss function $\ell_\gamma$ is differentiable with respect to $\theta$, so we can minimize it using first order methods.

\GLcomment{I think this sort of equivalence may hold for polynomial loss functions, but have not worked out the details.}


\subsection{Log Loss}
For log loss, we do not have a similar characterization as before. It is an interesting direction for future work to understand if it is possible to relate EasyLLP with the log loss, denoted $\losseasylog$, to other loss functions. In our experiments, we also consider the bag-level log loss function:
\begin{align*}
    \lossbaglog(f,B) \coloneqq - \alpha \cdot \log \prn*{\frac{\frac{1}{k} \sum_i f(x_i)}{\alpha}} - (1-\alpha) \cdot \log \prn*{ \frac{1 - \frac{1}{k} \sum_i f(x_i)}{1-\alpha}}.
\end{align*}

This loss is minimized whenever $\frac{1}{k}\sum_i f(x_i) \approx \alpha$, i.e., the proportions are matched.

\subsection{Relating Square Loss to EasyLLP}

\subsection{Proof Sketch}
\paragraph{Further background on square loss.} \GLcomment{to be reorganized.}The square loss rule was proposed in \cite{chen2023learning}. We consider a slightly modified version due to different assumptions on bag construction.
\begin{align*}
    \lossbagsq(f, B) &\coloneqq k \cdot \prn*{ \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 - \frac{1}{k} \sum_{i \ne j} \prn*{f(x_i) - p} \prn*{f(x_j) - p}.
\end{align*}

We can also show that $\lossbagsq$ is an unbiased estimate of the classification loss.
\begin{proposition}\label{prop:unbiased-sq}
For any predictor $f$, the loss $\lossbagsq(f, B)$ is an unbiased estimator of $\lossclass$.
\end{proposition}

\begin{proof}
We compute the expectation as follows.
\begin{align*}
    \En_{B} \lossbagsq(f, B) &\coloneqq \En_{B} \brk*{k \cdot \prn*{ \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2} - \En_B \brk*{\frac{1}{k} \sum_{i \ne j} (f(x_i) - p) (f(x_j) - p) }\\
    &\overset{(i)}{=} \frac{1}{k} \cdot \En_{B} \brk*{ \prn*{  \sum_{i} f(x_i) - y_i }^2} - (k-1) \prn*{\En f(x) - p}^2 \\
    &= \frac{1}{k} \cdot \En_{B} \brk*{ \sum_i (f(x_i) - y_i)^2 + \sum_{i \ne j} (f(x_i) - y_i)(f(x_j) - y_j) } - (k-1) \prn*{\En f(x) - p}^2 \\
    &\overset{(ii)}{=} \cL(f) + \frac{1}{k} \cdot \En_{B} \brk*{\sum_{i \ne j} (f(x_i) - y_i)(f(x_j) - y_j) } - (k-1) \prn*{\En f(x) - p}^2 \\
    &\overset{(iii)}{=} \cL(f).
\end{align*}
Equality $(i)$ follows from the fact that $\sum_{i} y_i = \alpha k$. Equality $(ii)$ uses the fact that for all $i$, $(f(x_i) - y_i)^2 = \ind{f(x_i) \ne y_i}$. Lastly, equality $(iii)$ uses the fact that for any $i \ne j$, by independence $\En_{B} \brk*{(f(x_i) - y_i)(f(x_j) - y_j) } = \En_{B} \brk*{f(x_i) - y_i} \En_{B} \brk*{f(x_j) - y_j } $.
\end{proof}

\paragraph{Reverse Square Loss.} We introduce a new bag-level loss function which we call the reverse square loss. Further intuition on it is deferred to the sequel.
\begin{align*}
\lossbagrsq(f, B) &\coloneqq 1 - k \cdot \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 + \frac{1}{k} \cdot \prn*{\sum_{i\ne j} (f(x_i) + p - 1)(f(x_j) + p - 1)}
\end{align*}


\begin{proposition}\label{prop:unbiased-rsq}
For any predictor $f$, the loss $\lossbagrsq(f, B)$ is an unbiased estimator of $\lossclass$.
\end{proposition}

\begin{proof}
We compute the expectation as follows:
\begin{align*}
    &\En_{B} \lossbagrsq(f, B) \\
    &= 1 - k \cdot 
    \En_B \brk*{ \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 } + \frac{1}{k} \cdot \En_B \brk*{\sum_{i\ne j} (f(x_i) + p - 1)(f(x_j) + p - 1) } \\
    &= 1 - k \cdot \En_B \brk*{ \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 } + (k-1) \prn*{\En f(x) + p - 1}^2 \\
    &= 1 - k + 2 \En_{B} \brk*{\sum_i f(x_i) + y_i} - \frac{1}{k} \En_{B} \brk*{\sum_i f(x_i)^2 + y_i^2 + 2 f(x_i) y_i + \sum_{i \ne j} (f(x_i) + y_i) \cdot (f(x_j) + y_j)} \\
    &\quad\quad\quad + (k-1) \prn*{\En f(x) + p}^2 - 2(k-1)\prn*{\En f(x) + p} + k-1 \\
    &\overset{(i)}{=} - \frac{2}{k} \cdot \En_{B} \brk*{\sum_i f(x_i)^2 + y_i^2} + \frac{1}{k} \En_{B} \brk*{\sum_i f(x_i)^2 + y_i^2 - 2 f(x_i) y_i - \sum_{i \ne j} (f(x_i) + y_i) \cdot (f(x_j) + y_j)} \\
    &\quad\quad\quad + (k-1) \prn*{\En f(x) + p}^2 + 2\prn*{\En f(x) + p} \\
    &\overset{(ii)}{=}  \frac{1}{k} \En_{B} \brk*{\sum_i f(x_i)^2 + y_i^2 - 2 f(x_i) y_i} =\frac{1}{k} \En_{B} \brk*{\sum_i (f(x_i) - y_i)^2} = \cL(f).
\end{align*}
In equality $(i)$ we use the fact that $f(x_i)^2 = f(x_i)$ and $y_i^2 = y_i$, in equality $(ii)$ we use independence and cancel out the extraneous terms as before.
\end{proof}

\paragraph{Expected Version of Losses.} In the sequel we will also consider \emph{expected} versions of the square loss and reverse square loss, where we replace the bias correction terms with their expectations. This has the effect of reducing the variance of the estimates. More formally, we define
\begin{align*}
    \wt{\lossbagsq}(f, B) &\coloneqq k \cdot \prn*{ \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 - (k-1) \prn*{\En f(x) - p}^2,\\
    \wt{\lossbagrsq}(f, B) &\coloneqq 1 - k \cdot \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 + (k-1) \prn*{\En f(x) + p - 1}^2.
\end{align*}

\begin{proposition}\label{prop:easyLLP-equivalence}
For any predictor $f$ and bag $B$, EasyLLP with classification loss can be written as
\begin{align*}
    \losseasyclass(f, B) = \frac{1}{2} \prn*{\lossbagsq(f, B) + \lossbagrsq(f, B)}.
\end{align*}
\end{proposition}

This equivalence only applies to $\lossbagsq$ and $\lossbagrsq$ and not their expected versions $\wt{\lossbagsq}$ and $\wt{\lossbagrsq}$.

\begin{proof}
This is a straightforward algebraic calculation. For notational convenience let us denote $\avgf \coloneqq \tfrac{1}{k} \sum_i f(x_i)$. Then we can rewrite the square loss estimator as
\begin{align*}
\lossbagsq(f, B) &= \underbrace{k\prn*{\avgf - \alpha}^2 - (k-1) \prn*{\avgf - p}^2}_{=: \mathbf{t}_1} + \underbrace{\frac{1}{k}\sum_{i} (f(x_i) - p)^2 - (\avgf - p)^2}_{=: \mathbf{t}_2}.
\end{align*}
Similarly the reverse square loss can be written as
\begin{align*}
    \lossbagrsq(f, B) &= \underbrace{1 - k \cdot \prn*{1 - \avgf - \alpha}^2 + (k-1) \prn*{ \avgf + p - 1}^2}_{=: \mathbf{t}_3} + \underbrace{ \prn*{\avgf + p - 1} - \frac{1}{k} \sum_i \prn*{f(x_i) + p - 1}^2 }_{=: \mathbf{t}_4}.
\end{align*}
From here we claim that:
\begin{align*}
    {\mathbf{t}_1} + {\mathbf{t}_3} = 2\losseasyclass(f, B), \quad \text{and} \quad \mathbf{t}_2 + \mathbf{t}_4 = 0,
\end{align*}
from which the conclusion of \pref{prop:easyLLP-equivalence} follows.

Now we show ${\mathbf{t}_1} + {\mathbf{t}_3} = 2\losseasyclass(f, B)$. Expanding the squares, we get
\begin{align*}
    {\mathbf{t}_1} + {\mathbf{t}_3} &= k \avgf^2 - 2k\avgf \alpha + k \alpha^2 - (k-1) \avgf^2 + 2(k-1) \avgf p  - (k-1) p^2 \\
    &\quad\quad + 1 - k - k \avgf^2 - k \alpha^2 + 2k \avgf + 2k \alpha - 2k \avgf\alpha \\
    &\quad\quad + (k-1) \avgf^2 + (k-1)p^2 + (k-1) + 2(k-1) \avgf p - 2(k-1) \avgf - 2(k-1) p,
\end{align*}
and further simplifying we get
\begin{align*}
    {\mathbf{t}_1} + {\mathbf{t}_3} &= -4k\avgf \alpha + 4(k-1) \avgf p + 2k \avgf + 2k \alpha - 2(k-1) \avgf - 2(k-1) p \\
    &= 2\cdot \prn*{\prn*{k(\alpha - p) + p} (1-\avgf) + \prn*{k(p - \alpha) + (1-p)} \avgf} \\
    &= 2\losseasyclass(f, B).
\end{align*}

Now we show that $\mathbf{t}_2 + \mathbf{t}_4 = 0$. This is straightforward after observing the identity 
\begin{align*}
    \prn*{(a-b)^2 - (a+b-1)^2} = 2a+2b  - 4ab - 2,
\end{align*}
and applying it separately to the terms in the summation. This concludes the proof of \pref{prop:easyLLP-equivalence}.
% Therefore, we get that
% \begin{align*}
% \mathbf{t}_2 + \mathbf{t}_4 \\
% =~&\frac{1}{k}\sum_{i} \prn*{f(x_i) - p}^2 - \prn*{\frac{1}{k}\sum_i f(x_i) - p}^2 + \prn*{\frac{1}{k}\sum_i f(x_i) + p - 1}^2 - \frac{1}{k} \sum_i \prn*{f(x_i) + p - 1}^2 \\
% =~& \frac{2}{k} \sum_i 
% \prn*{f(x_i) + p - 2f(x_i) p - 1} - \frac{2}{k} \sum_i 
% \prn*{f(x_i) + p - 2f(x_i) p - 1} = 0.
% \end{align*}
\end{proof}

\subsection{Example: 1D Linear Classification with Random Classification Noise}

To provide some intuition on these learning rules, we will study a simple setting. Let the instance space $\cX = \crl{0,1}$. We consider a family of distributions $\cD_\eta$ parameterized by $\eta \in [0,1]$ where $\cD_\eta$ is defined as
\begin{align*}
    x \sim \unif(\crl{0,1}), \quad y = \begin{cases}
        x &\text{w.p.}~1-\eta,\\
        1-x &\text{w.p.}~\eta.
    \end{cases}
\end{align*}

\paragraph{Estimation of Bayes-Optimal Predictor.} Consider the predictor $f^\star(x) = x$, which in the regime $\eta \in [0, 1/2]$ is the Bayes-optimal predictor. The classification loss of $f^\star$ in $\cD_\eta$ is $\cL(f^\star) = \eta$. From the previous section, we know that all three aggregate learning rules $\losseasyclass, \lossbagsq, \lossbagrsq$ are unbiased estimates of $\cL$. However, for any fixed bag, the loss functions output different values.

Fix a bag $B = \crl{x_1, \cdots, x_k, \alpha}$. For notational convenience we consider the quantities 
\begin{align*}
   n_x \coloneqq \sum_{i=1}^k x_i, \quad\text{and}\quad n_y \coloneqq k\alpha.
\end{align*}
The quantities $n_x$ and $n_y$ include all relevant information about the bag $B$. Note that in this case, we exactly know the distribution of $(n_x, n_y)$:
\begin{align*}
    n_x \sim \bin(k, 1/2), \quad\text{and}\quad
    n_y \sim \bin(n_x, 1-\eta) + \bin(k-n_x, \eta).
\end{align*}

We rewrite $\ell_{\square}(f^\star,B)$ as a function of $n_x$ and $n_y$ for $\square \in \crl{\mathsf{easy.01}, \mathsf{bag.sq}, \mathsf{bag.rsq}}$:
\begin{align*}
    \losseasyclass(f^\star, B) &= n_x + n_y - \frac{2}{k} \cdot n_x n_y - \frac{k}{2} + \frac{1}{2}, \\
    \lossbagsq(f^\star, B) &= \frac{1}{k} \cdot \prn*{n_x - n_y}^2 - \frac{1}{k} \cdot \prn*{n_x - \frac{k}{2}}^2 + \frac{1}{4}, \\
    \lossbagrsq(f^\star, B) &= 1 - \frac{1}{k}\cdot \prn*{n_x + n_y - k}^2 + \frac{1}{k} \cdot \prn*{n_x - \frac{k}{2}}^2 - \frac{1}{4}.
\end{align*}
We also have for the expected versions of square and reverse square
\begin{align*}
    \wt{\lossbagsq}(f^\star, B) &= \frac{1}{k} \cdot \prn*{n_x - n_y}^2, \\
    \wt{\lossbagrsq}(f^\star, B) &= 1 - \frac{1}{k}\cdot \prn*{n_x + n_y - k}^2.
\end{align*}
In this setting, we have the equivalence $\losseasyclass = \frac{1}{2} \prn*{\wt\lossbagsq + \wt\lossbagrsq}$; in general, this is not true.

To tease out the differences, let us consider the extremes $\eta = 0$ and $\eta = 1$. We will focus on the differences between $\losseasyclass, \wt\lossbagsq, \wt\lossbagrsq$. 
\begin{itemize}
    \item When $\eta = 0$, we always have $n_x = n_y$, so $\wt\lossbagsq(f^\star, B) = 0$, while $\wt\lossbagrsq(f^\star, B) = 1 - \frac{1}{k} (2n_x - k)^2$, which is a random variable that has expectation 0. Similarly $\losseasyclass(f^\star, B) =  \frac{1}{2} - \frac{1}{2k} (2n_x - k)^2$ is also a random variable that has expectation 0.
    \item When $\eta = 1$, we always have $n_x = k-n_y$, and the reverse is true: $\wt\lossbagrsq(f^\star, B) = 1$ while $\wt\lossbagsq(f^\star, B)$ and $\losseasyclass(f^\star, B)$ are random variables which have expectation 1.
\end{itemize}
\GLcomment{For the original loss functions $\lossbagsq$ and $\lossbagrsq$, this behavior does not hold, since the loss is random at both $\eta = 0$ and $\eta = 1$, but it is still true that the variances have a similar asymmetric behavior, as shown in \pref{fig:mean-variance}.}


\begin{figure}[!t]
    \centering
\includegraphics[scale=0.45, trim={0cm 0cm 0cm 0cm}, clip]{figures/mean-variance.png}
\caption{We generate bags according to $\cD_\eta$ for varying $\eta \in [0,1]$ and plot the empirical mean and variance of the loss estimates of $f^\star$ for various estimators. The loss estimate curves are plotted using $N = 10^6$ bags, while the Cramer-Rao lower bound is estimated with $N=10^4$ bags.}
\label{fig:mean-variance}
\end{figure}

More generally, we can plot the mean and variance of these estimators under consideration as we vary $\eta$. This is done in \pref{fig:mean-variance}. As expected, each estimator is an unbiased estimate of the true loss $\cL(f^\star)$ (as shown on the left). However, the variance of each estimate is drastically different, as shown in the middle plot. The estimator $\wt\lossbagsq$ has near zero variance when $\eta \approx 0$ and high variance when $\eta \approx 1$, while $\wt\lossbagrsq$ has the opposite behavior. Since $\losseasyclass$ is an average of $\wt\lossbagsq$ and $\wt\lossbagrsq$, it has nonzero variance across the entire range $\eta \in [0,1]$. Similar, although less pronounced behavior can be seen in the right plot which shows the variance of $\lossbagsq$ and $\lossbagrsq$ instead.

\GLcomment{Not sure how to present this.} We also comment on the other curves in the figure.
\begin{itemize}
    \item The red curve is associated with a new \emph{two-step estimator}, which attempts to get the best performance across the entire range of $\eta$. Notice that any estimate of the form $(1-\beta) \wt\lossbagsq + \beta \wt\lossbagrsq$ is an unbiased estimate of the classification loss. For any predictor $f$ and bag $B$ we define:
    \begin{align*}
        \lossbagtwostep(f, B) \coloneqq \prn*{1- \hat{\ell}(f)} \wt\lossbagsq(f, B) + \hat{\ell}(f) \wt\lossbagrsq(f, B).
    \end{align*}
    Here $\hat{\ell}(f)$ is an estimate of the loss of $f$, which can be obtained by using the EasyLLP on a held-out dataset, for example. In the figure, we use EasyLLP on the same dataset, and empirically we observe little bias caused by this.
    \item The purple dashed line plots an estimate of the Cramer-Rao lower bound, which is:
    \begin{align*}
        \mathsf{CR}(\eta) \coloneqq \En_{B \sim \cD_\eta} \brk*{\prn*{\frac{d\log q(B; \eta)}{d\eta}}^2}^{-1},
    \end{align*}
    where $q(B; \eta)$ is the likelihood function which is
    \begin{align*}
        q(B; \eta) \coloneqq \sum_{j = \max\crl{n_y - n_x, 0}}^{\min\crl{n_y, k-n_x}} {k-n_x \choose j } {n_x \choose n_y - j} p^{n_x - n_y + 2j} (1-p)^{k - n_x + n_y - 2j}.
    \end{align*}
    We observe that for all values of $\eta$, the two-step estimator's variance is close to that of the Cramer-Rao lower bound, which is the minimum variance of any unbiased estimator.
\end{itemize}

\GLcomment{(1) Can we prove with $\wh{\ell} \coloneqq \eta$ the estimator is close to the CR lower bound? (2) Is there a different choice of averaging function that gets closer to the CR lower bound? For example, we can try to match the derivatives at 0 and 1.}

\paragraph{Main Takeaway.} The behavior of the expected vs unexpected versions of the square loss and reverse square loss can be different. To use the two-step estimator, it seems better to average the expected versions $\wt\lossbagsq$ and $\wt\lossbagrsq$ instead of of $\lossbagsq$ and $\lossbagrsq$, as the variance is drastically reduced.

\section{Attempt: Slow Rates for EasyLLP}
\begin{theorem}[Slow Rates for EasyLLP]\label{thm:slow-easyllp}
For bag size $k = 3$ and $\eps \in (0, 1)$, there exists a function class $\cF$ with $\VC(\cF) = 1$ and distribution $\cD$ which satisfies $\inf_{f \in \cF} \cL(f) = 0$ such that the EasyLLP learning rule requires at least $\Omega(\log(1/\eps)/\eps)$ samples in order to return an $\eps$-optimal predictor with constant probability.
\end{theorem}

\GLcomment{unfortunately, proving a $\Omega(\log(1/\eps)/\eps)$ is not super interesting. It is already known for proper learners in the standard classification setting, and we know that when $k=1$, EasyLLP is a proper learning rule.}


\paragraph{Lower Bound Construction.}
For the lower bound, we will construct an input space $\cX$, function class $\cF \subseteq \crl{0,1}^\cX$, as well as a distribution $\cD$. The construction depends on the parameter $\eps$ which is specified.

Let $M = 1/(2\eps)$. \GLcomment{for simplicity we assume $M$ is an integer.} We define the input space $\cX = \crl*{x_0, x_1, \cdots, x_M}$. We define the function class $\cF = \crl{f_0, f_1, \cdots, f_M}$, where
\begin{align*}
    f_0(x) = \ind{x = x_0}, \quad \text{and} \quad f_i(x) = \ind{x \in \crl*{x_0, x_i}} ~\text{for all}~i \in [M].
\end{align*}
It is easy to check that $\VC(\cF) = 1$.

For the distribution $\cD$, we set:
\begin{align*}
\cD = \begin{cases}
    (x_0, 1) &\text{w.p.}~\frac{1}{2}, \\
    (x_i, 0) &\text{w.p.}~ \eps, ~ \text{for all }i \in [M].
\end{cases}
\end{align*}
One can check that under $\cD$, $f_0$ is the optimal predictor which achieves 0 classification error, and every $f_i$ is $\eps$-suboptimal.

Lastly, we observe that $p = \Pr\brk*{Y=1} = 0.5$.

\paragraph{EasyLLP Loss Predictions.} Given a dataset of bags $\crl*{(B_t, \alpha_t)}_{t\in[n]}$, we can explicitly compute the form of the EasyLLP estimates. For a bag $B$, we define $(\beta_0, \beta_1, \cdots, \beta_M)$ to be the empirical proportion of number of points.

For the function $f_0$, we have
\begin{align*}
    \wh{L}(f_0) &= \frac{1}{n} \sum_{t=1}^n \crl*{ \prn*{k(\alpha_t - 1/2) + 1/2} \cdot \prn*{\sum_{j \ge 1} \beta_{t,j} } + \prn*{k(1/2 - \alpha_t) + 1/2} \cdot \prn*{1 - \sum_{j \ge 1} \beta_{t,j} } } \\
    &= \frac{1}{n} \sum_{t=1}^n \crl*{ k\cdot \prn*{1/2 - \alpha_t} + 1/2 + k \prn*{2\alpha_t - 1} \cdot \prn*{\sum_{i \ge 1} \beta_{t,j} }  }
\end{align*}
Likewise for any $f_i$, $i\in [M]$ the EasyLLP estimate is
\begin{align*}
    \wh{L}(f_i) &= \frac{1}{n} \sum_{t=1}^n \crl*{ \prn*{k(\alpha_t - 1/2) + 1/2} \cdot \prn*{- \beta_{t,i} + \sum_{j \ge 1} \beta_{t,j} } + \prn*{k(1/2 - \alpha_t) + 1/2} \cdot \prn*{1 + \beta_{t,i} - \sum_{j \ge 1} \beta_{t,j} } } \\
    &= \frac{1}{n} \sum_{t=1}^n \crl*{ k\cdot \prn*{1/2 - \alpha_t} + 1/2 + k \prn*{2\alpha_t - 1} \cdot \prn*{-\beta_{t,i} + \sum_{i \ge 1} \beta_{t,j} }  }
\end{align*}

For every $i \in [M]$, we will also define the errors:
\begin{align}
    \Delta_i(B, \alpha) \coloneqq \beta_{i}k (1-2\alpha),
\end{align}
so that $\wh{L}(f_i) = \wh{L}(f_0) + \frac{1}{n} \sum_{t=1}^n \Delta_i(B_t, \alpha_t)$.

Let us fix $k=3$. \GLcomment{this is the smallest $k$ for which I think the lower bound works.} We can explicitly write out the distribution of $\Delta_i(\beta, \alpha)$ (which is the same for all $i$).

\begin{align*}
    \Delta_i(\beta, \alpha) = \cdot \begin{cases}
        -1/3 &\text{w.p.}~3/4 \cdot \eps \\
        1/3 &\text{w.p.}~3/2 \cdot \eps(1-2\eps) \\
        2/3 &\text{w.p.}~3/2 \cdot \eps^2\\
        1 &\text{w.p.}~3/4 \cdot \eps (1-2\eps)^2\\
        2 &\text{w.p.}~3/2 \cdot \eps^2(1-2\eps) \\
        3 &\text{w.p.}~\eps^3\\
        0 &\text{otherwise.}
    \end{cases}
\end{align*}
We can check that $\En \Delta_i(B, \alpha) = \eps$. We want show that
\begin{align*}
    \Pr\brk*{\exists i \in [M]: \sum_t \Delta_i(B_t, \alpha_t) \le 0} \ge \Omega(1).
\end{align*}

\paragraph{Lower Bound Argument.} Thus, our task is to show that with constant probability, there exists some $i \in [M]$ such that the term $\frac{1}{n} \sum_{t=1}^n \Delta_i(B_t, \alpha_t) \le 0$, and therefore $\wh{f}_i$ will be returned by the EasyLLP learning rule. Since $\wh{f}_i$ is $\eps$-suboptimal, this proves the result.

We will define the two events:
\begin{align*}
    \cE_1 &\coloneqq \crl*{\exists i \in [M]: \frac{1}{n} \sum_{t=1}^n \ind{\Delta_i(B_t, \alpha_t) = -1/3} \ge \frac{Cn}{M} } \\
    \cE_2 &\coloneqq \crl*{\forall i \in [M]: \frac{1}{n} \sum_{t=1}^n \ind{\Delta_i(B_t, \alpha_t) \ne 0} \le 4\epsilon}.
\end{align*}

We pick $n = \frac{1}{4} \cdot \log (1/2\eps) /2\eps = O(\log(1/\eps)/\eps)$, where $c > 0$ is an absolute numerical constant. By Paley-Zygmund (\pref{thm:paley-zygmund}), we have
\begin{align*}
    \Pr \brk*{\sum_{t=1}^n \ind{\alpha_t = 2/3} \ge 0.9 \cdot \frac{3n}{8} } \ge 0.01 \cdot \frac{9n^2/64}{15n/64+9n^2/64} \ge 0.01 \cdot \frac{3}{8}.
\end{align*}
Let us denote the set $N_b \subset [N]$ to be $N_b \coloneqq \crl*{t \in [n]: \alpha_t = 2/3}$. With constant probability we know that $N_b \ge 0.9 \cdot 3n/8$. Observe that once we condition on $t \in N_b$, the probability that $\Delta_i(B_t, 2/3) = -1/3$ is exactly $\eps$, and the distribution of $\sum_{t \in N_b} \Delta_i(B_t, 2/3)$ for every $i$ is given by the balls into bins problem where we are throwing $\abs{N_b}$ balls into $M  = 1/(2\eps)$ bins.

In fact we will only consider the first $n_{b} \coloneqq 0.9 \cdot 3n/8$ such $t \in N_b$. Now we can apply \pref{thm:balls-in-bins} to show that with constant probability, event $\cE_1$ holds. Let $C >0$ be some absolute numerical constant to be determined later. We see that
\begin{align*}
    \Pr \brk*{\exists i \in [M]: \sum_{t\in n} \ind{\Delta_i(B_t, \alpha_t) = -1/3} \ge \frac{Cn}{M}} &\ge \Pr \brk*{\exists i \in [M]: \sum_{t\in N_{b}} \ind{\Delta_i(B_t, \alpha_t) = -1/3} \ge \frac{Cn}{M}} \\
    &\ge 1 - \exp \prn*{- \frac{Cn}{M} \cdot \prn*{\rho_{n_{b}, Cn/M} - \log \rho_{n_{b}, Cn/M} - 1}},
\end{align*}
provided that the condition $\rho_{n_{b}, Cn/M} > 1$ holds.
Now we prove a lower bound on $\rho_{n_{b}, Cn/M}$. We can write
\begin{align*}
    \rho_{n_{b}, Cn/M} = \frac{n_b \cdot M^{M/Cn}}{M \cdot Cn/M} = \frac{0.9 \cdot 3/8}{C} \cdot \prn*{\frac{1}{2\eps}}^{600/C \log(1/2\eps)} \ge 1.36,
\end{align*}
where we pick $C$ to be a suitably large constant like $100$.
so that we have
\begin{align*}
    \Pr \brk*{\exists i \in [M]: \sum_{t\in n} \ind{\Delta_i(B_t, \alpha_t) = -1/3} \ge \frac{Cn}{M}} &\ge 1 - \exp \prn*{- 1/100 \log (1/\eps)} = 1 - \eps^{1/100},
\end{align*}
which for sufficiently small $\eps$ is at least $0.1$.

Thus we can conclude that $\cE_1$ holds with probability at least $\Omega(1)$.

Also, by Chernoff Bounds, it is easy to see that $\cE_2$ holds with probability $0.999$. So $\cE_1 \cup \cE_2$ holds with constant probability.



\subsection{Technical Lemmas}
Consider the balls into bins problem of throwing $n$ balls into $m\ge 2$ bins.

\begin{theorem}[Cor.~1 of \cite{schulte2022balls}]\label{thm:balls-in-bins} Let $B_n$ denote the maximum load of throwing $n$ balls into $m$ bins. For any $k \ge 1$, let $\rho_{n,k} \coloneqq \frac{nm^{1/k}}{mk}$. Then if $\rho_{n,k} > 1$ we have
\begin{align*}
    \Pr \brk*{B_n \ge k} \ge 1 - \exp\prn*{-k \cdot \prn*{\rho_{n,k} - \log  \rho_{n,k} - 1}}.
\end{align*}
\end{theorem}

\begin{theorem}[Paley-Zygmund]\label{thm:paley-zygmund}
Let $Z \ge 0$ be a random variable with finite variance. For any $\theta \in [0,1]$,
\begin{align*}
    \Pr\brk*{Z \ge \theta \cdot \En Z} \ge (1-\theta)^2 \frac{\En[Z]^2}{\En [Z^2]}.
\end{align*}
\end{theorem}

\begin{theorem}[Chernoff Bounds]
Let $X_1, \cdots, X_n$ be i.i.d random variables taking values in $\crl{0,1}$. Then for any $\delta \ge 0$,
\begin{align*}
    \Pr \brk*{\frac{1}{n} \sum_i X_i \ge (1+\delta) \En X} \le \exp \prn*{\frac{-\delta^2 n \En X}{2 + \delta}}.
\end{align*}
\end{theorem}

% \section{Surrogate Losses}

% \subsection{Square Loss}
% Now we allow $\cF \subseteq \bbR^\cX$ and consider the instance-level square loss $\ell(f,(x,y)) = \prn{f(x) - y}^2$. The question now is whether we again write the EasyLLP estimator as average of two losses. Inspecting the proof of \pref{prop:unbiased-sq}, we can notice that $\ell_\mathrm{sq}(f, B)$ is still unbiased. That is, $\En_B \ell_\mathrm{sq}(f, B) = \En (f(x) - y)^2$ still holds.

% However in the proof of \pref{prop:unbiased-rsq} we heavily relied on the fact that $f(x) = f(x)^2$ for $f \in \crl{0,1}^\cX$; when $f$ is real-valued, this is equality is not satisfied. 

% We can slightly modify the definition of the reverse square loss by adding a factor of 
% \begin{align*}
%     \frac{2}{k} \prn*{\sum_i f(x_i)^2 - f(x_i)}
% \end{align*} to it. Notice that when $f(x) \in \crl{0,1}$, this additional term is zero. However, when $f(x) \in \bbR$, the effect of the last term is to correct the $\sum_i f(x_i)$ when expanding the square to become $\sum_i f(x_i)^2$. In this way, we can show that $\ell_\mathrm{rsq}(f, B)$ remains an unbiased estimate of the instance-level square loss. One can also replace the last term with its expectation, i.e., $2 \En \brk*{ f^2 - f}$. The effect of the last term is to encourage $f$ to predict values that lie in the range $[0,1]$.

% We have the following proposition.
% \begin{proposition}
% Consider the loss function $\ell(f,(x,y)) = \prn{f(x) - y}^2$. Define the respective square and reverse square losses as
% \begin{align*}
%     \ell_\mathrm{sq}(f, B) &\coloneqq k \cdot \prn*{ \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 - \frac{1}{k} \sum_{i \ne j} (f(x_i) - p) (f(x_j) - p)\\
%     \ell_\mathrm{rsq}(f, B) &\coloneqq 1 - k \cdot \prn*{1- \frac{1}{k} \sum_{i} f(x_i) - \alpha }^2 + \frac{1}{k} \cdot \prn*{\sum_{i\ne j} (f(x_i) + p - 1)(f(x_j) + p - 1)} \\
%     &\quad\quad\quad + \frac{2}{k} \prn*{\sum_i f(x_i)^2 - f(x_i)}.
% \end{align*}
% Then we have 
% \begin{align*}
%     \ell_\mathrm{easy} = \frac{1}{2} \prn*{\ell_\mathrm{sq}(f, B) + \ell_\mathrm{rsq}(f, B)}.
% \end{align*}
% \end{proposition}


% With the square loss, we naturally have an algorithmic approach to solve classifcation in aggregate learning. Let $\cF_\Theta = \crl{f_\theta: \theta \in \Theta}$ be a continuously parameterized function class. Consider the loss function:
% $\ell_\gamma(f_\theta, B) = (1-\gamma) \ell_\mathrm{sq}(f_\theta, B) + \gamma \ell_\mathrm{rsq}(f_\theta, B)$. EasyLLP corresponds to picking $\gamma = 1/2$. However, we can pick other choices of $\gamma$. Our intuition says that $\gamma$ should be small if we are realizable, since the variance of this estimate is reduced. The loss function $\ell_\gamma$ is differentiable with respect to $\theta$, so we can minimize it using SGD.

% \GLcomment{Does this equivalence hold for general $\ell_p$ losses?}

% \clearpage
% \subsection{Log Loss}
% \GLcomment{This section is more speculative.}
% Consider the EasyLLP learning rule using log loss, i.e., 
% \begin{align*}
%     \ell(f, (x,y)) \coloneqq -\brk*{y \log f(x) + (1-y) \log (1- f(x))}.
% \end{align*}

% \paragraph{Simple Case.} Let's think about the simple case of 1D classification with RCN. Consider the function 
% \begin{align*}
%     f(x) = \begin{cases}
%        v_+ &\text{if}~ x=1\\
%        v_- = 1-v_+ &\text{if}~ x=-1.
%     \end{cases} 
% \end{align*}
% Let us denote $\wt{v}_+ = -\log v_+$ and $\wt{v}_- = -\log v_-$. Use $\alpha_x$ to denote the fraction of $+1$s in a bag and $\alpha_y$ to denote the fraction of $-1$ in a bag. Then we have the estimate
% \begin{align*}
%     \ell_\mathrm{easy}(f, B) &= \prn*{k(\alpha_y - 1/2) + 1/2}\prn*{\alpha_x \cdot \wt{v}_+ + (1-\alpha_x) \wt{v}_-} + \prn*{k(1/2 - \alpha_y) + 1/2}\prn*{\alpha_x \cdot \wt{v}_- + (1-\alpha_x) \wt{v}_+}\\
%     &= \prn*{- k \alpha_x  - k\alpha_y + 2k \alpha_x \alpha_y   + \frac{k}{2}  + \frac{1}{2}  } \cdot \wt{v}_+ + \prn*{k \alpha_x  + k\alpha_y - 2k \alpha_x \alpha_y   - \frac{k}{2}  + \frac{1}{2}  }\cdot \wt{v}_-. 
% \end{align*}
% In the classification case, this corresponded to having $\wt{v}_+ = 0$ and $\wt{v}_- = 1$. So one can write this as a combination of square losses. However, it seems difficult to generalize this to more interesting scenarios. \GLcomment{The problem is that it is hard to see what happens with more general $f$.}


\section{EasyLLP Learning Rule}
Consider the hypothesis class consisting of linear predictors.
\begin{align*}
    \cH \coloneqq \crl*{x \mapsto \ind{w^\top x \ge 0}: w \in \bbR^d}.
\end{align*}
In this section, we will use the convention that $n$ is the total number of samples and $k$ is the bag size, so that the total number of bags we get is $n/k$.

Now we will see what happens when we apply the EasyLLP algorithm. The EasyLLP algorithm first generates labels $\wt{y}_{i1}, \cdots, \wt{y}_{ik} \sim \mathrm{Ber}(\alpha_i)$ for each sample. At this point, one can run the ERM algorithm:
\begin{align*}
    \wh{w} = \argmin_{w} \frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k \ell^{01}(w, (x_{ij}, \wt{y}_{ij})).
\end{align*}
However, as remarked in \cite{busa2023easy}, this is a biased estimator for $L(w) \coloneqq \En_{(x,y)\sim \cD}\brk{\ell^{01}(w,(x,y))}$.

Specifically let us calculate the bias (this calculation is already in their paper). We will fix $i,j$ and drop the index $i$. Also let $p \coloneqq \Pr\brk{y=1}$.
\begin{align*}
    \En \brk*{\ell^{01}(w, (x_{j}, \wt{y}_{j}))} &= \frac{1}{k} \sum_{j'=1}^k \En \brk*{ \ell^{01}(w, (x_{j}, y_{j'})) } \\
    &= \frac{1}{k} \En \brk*{ \ell^{01}(w, (x_{j}, y_{j})) } + \frac{1}{k}\sum_{j' \ne j} \En \brk*{ \ell^{01}(w, (x_{j}, y_{j'})) } \\
    &= \frac{1}{k} \En \brk*{ \ell^{01}(w, (x_{j}, y_{j})) } + \frac{k-1}{k} \prn*{(1-p) \cdot \En\brk*{ \ell^{01}(w, (x, 0 )) } + p \cdot \En\brk*{ \ell^{01}(w, (x, +1 )) }}
\end{align*}
So actually we should use the learning rule
\begin{align*}
    \wh{w}_\mathrm{surr} &= \argmin_{w} \frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k k \cdot \ell^{01}(w, (x_{ij}, \wt{y}_{ij})) - (k-1) \cdot \prn*{(1-p) \cdot \ell^{01}(w, (x_{ij}, 0))  + p \cdot \ell^{01}(w, (x_{ij}, +1 )) } \\
    &= \argmin_{w} \frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k \underbrace{ \prn*{k(\wt{y}_{ij} - p) + p}  \ell^{01}(w, (x_{ij}, +1 )) + \prn*{k(p - \wt{y}_{ij}) + (1-p)} \ell^{01}(w, (x_{ij}, 0 )) }_{\ell_\mathrm{surr}}.
\end{align*}
By the above calculation, this learning rule is unbiased and uses $O(k^2/\eps^2)$ samples, since each term is on the order of $O(k)$. They also propose another estimator which reduces the variance to get sample complexity $O(k/\eps^2)$.

We will consider the following estimator which directly uses the label proportions. It is also unbiased.
\begin{align*}
   \wh{w}_\mathrm{easy} &= \argmin_{w} \frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k \underbrace{ \prn*{k(\alpha_i - p) + p}  \ell^{01}(w, (x_{ij}, +1 )) + \prn*{k(p - \alpha_i) + (1-p)} \ell^{01}(w, (x_{ij}, 0 )) }_{\ell_\mathrm{easy}}
\end{align*}

\paragraph{Variance Calculations.}
First we calculate the variance of the surrogate estimator. Here is a trivial upper bound. \GLcomment{this probably cannot be improved that much.}
\begin{proposition}
    $\mathrm{Var}(\ell_\mathrm{surr}) \le \max \crl*{k(1-p) + p, kp + (1-p)}^2 \le k^2$.
\end{proposition}
\GLcomment{The increase in variance can be seen by looking at the proof for the below proposition, which uses an intermediate quantity $A = y_i + B$ where $B$ is a centered binomial. If we use the surrogate loss, the intermediate quantity becomes $A' = y_i + B + k(\wt{y} - \alpha)$, so we do not get a concentration effect due to the additional last term, since it is just a single Bernoulli.}

The EasyLLP estimator has variance which is only $O(k)$.
\begin{proposition}
    $\mathrm{Var}(\ell_\mathrm{easy}) \le 4 + (k-1) p (1-p)$.
\end{proposition}
As a consequence, by Bernstein's inequality, the EasyLLP estimator only uses at most $n = O(k/\eps^2)$ samples.

\paragraph{Does the uncorrected estimator fail?} For any predictor $w$ let us use $p_w \coloneqq \Pr[h_w(x) = +1]$ (i.e., the marginal probability over the data that the predictor $w$ predicts a label of $1$).
In the population limit the uncorrected estimator converges to the solution
\begin{align*}
    w^\star &\coloneqq \argmin_{w} \En \brk*{ \ell^{01}(w, (x_{j}, y_{j})) } + (k-1) \prn*{(1-p) \cdot \En\brk*{ \ell^{01}(w, (x, 0 )) } + p \cdot \En\brk*{ \ell^{01}(w, (x, +1 )) }} \\
    &= \argmin_{w} \En \brk*{ \ell^{01}(w, (x_{j}, y_{j})) } + (k-1) \prn*{(1-p) p_w + p (1-p_w) }.
\end{align*}
That is, there is an additional term $(k-1) \prn*{(1-p) p_w + p (1-p_w) }$. Let us investigate what the minimizer of this is by itself.
\begin{align*}
    \argmin_{p_w \in [0,1]} \quad (1-p) p_w + p (1-p_w) = \ind{p \ge 1/2}.
\end{align*}
Due to the pre-factor of $(k-1)$, it is conceivable that the second term greatly dominates the first term, so we might not even have consistency of the uncorrected loss. Consider some construction as follows:
\begin{align*}
    \cD \coloneqq \begin{cases}
        (x = +1, y = +1) &\text{w.p.}~1/2 + \gamma. \\
        (x = -1, y = 0) &\text{w.p.}~1/2 - \gamma.
    \end{cases}
\end{align*}
The error here of the uncorrected estimator can be $\Omega(1)$. Consider the two possibilities.
\begin{enumerate}
    \item Classify everything as positive. Then the population value is $1/2-\gamma$.
    \item Classify the +1 points as positive and the -1 points as negative. Then the population value is $2(k-1)(1/2-\gamma)(1/2+\gamma) \approx (k-1)/4$.
\end{enumerate}
The uncorrected estimator will return the first choice.

\paragraph{Discussion.}
It seems like the surrogate approach cannot attain the optimal $O(1/\eps)$ rate. First, it has a dependence on $k$, and it cannot adapt to realizability of the instance. In general, it might be interesting to study when one can get fast rates under realizability for aggregate learning.

Now we also prove a generalization guarantee for the EasyLLP learning rule \cite{busa2023easy} for VC classes. Recall that the EasyLLP learning returns the following hypothesis
\begin{align*}
    \wh{f} \gets \argmin_{f \in \cF} \frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k \wt{\ell}(f(x_{ij}), \alpha_i),
\end{align*}
where $\wt{\ell}(f(x), \alpha) \coloneqq \prn*{k(\alpha - p) + p} \ell^{01}(f(x), 1) + \prn*{k(p - \alpha) + (1-p)} \ell^{01}(f(x), 0)$. 

Another way to write the bag level loss of a predictor $f$ is as:
\begin{align*}
    \wh{\ell}(f, \alpha) &\coloneqq \frac{1}{k} \sum_{j=1}^k \prn*{k(\alpha - p) + p} (1-f(x_j)) + \prn*{k(p - \alpha) + (1-p)} f(x_j) \\
    &= \frac{1}{k} \sum_{j=1}^k -\prn*{k(\alpha - p) + p} f(x_j) + \prn*{k(p-\alpha) + (1-p) } f(x_j) +\prn*{k(\alpha - p) + p} \\
    &= \frac{1}{k} \sum_{j=1}^k \prn*{2k(p - \alpha) + 1-2p} f(x_j) + \prn*{k(\alpha - p) + p} \\
    &= \prn*{2(p - \alpha) + \frac{1-2p}{k}} \prn*{\sum_{j=1}^k f(x_j)} + \prn*{k(\alpha - p) + p} \numberthis
\end{align*}
The first inequality follows from the fact that when $f(x) \in \crl{0,1}$, we have $\ell^{01}(f(x), 0) = \ind{f(x) \ne 0} = f(x)$, and similarly $\ell^{01}(f(x), 1) = \ind{f(x) \ne 1} = (1-f(x))$.

One way to think about this is that the loss is a linear function of the average prediction that $f$ makes on the bag. \GLcomment{This still looks mysterious to me.}

\subsection{Generalization Guarantee}
We have the following theorem:
\begin{theorem}
The EasyLLP learning rule uses $O(\VC(\cF) k^2 \log k/ \eps^2)$ samples to return an $\eps$-optimal predictor.
\end{theorem}

\begin{proof}
By the results in \cite{busa2023easy}, the quantity $\wt{\ell}(f(x), \alpha)$ is a consistent estimator for $\cL(f)$. Our aim is to prove a uniform convergence guarantee that shows the empirical estimate converges to $\cL(f)$ for all $f \in \cF$.

Let us define the loss function and class:
\begin{align*}
    \wt{\ell}_B(f) &\coloneqq \frac{1}{k} \sum_{j} \prn*{k(\alpha - p) + p} \ell^{01}(f(x), 0) + \prn*{k(p - \alpha) + (1-p)} \ell^{01}(f(x), 1)
    \\ \cF_\cB &\coloneqq \crl{B \mapsto \wt{\ell}_B(f): f \in \cF} \subseteq \brk{-k, k}^B.
\end{align*}

Now we will calculate the VC subgraph dimension. Define the class $\cF_\cB^{+} : \cB \times \bbR \to \crl{0,1}$ to be the subgraph class. Then we can calculate the VC subgraph dimension as $\VC(\cF_\cB^{+})$. Using similar reasoning as before, we can compute that
\begin{align*}
    \VC(\cF_\cB^{+}) \le O(\VC(\cF) \log k).
\end{align*}
This is again due to the fact that among a sample of $d$ bags (with $dk$ examples), the total number of behaviors is upper bounded by $(dk)^{\VC(\cF)}$.

Thus, we can arrive at the generalization guarantee:
\begin{align*}
    \Pr_S\brk*{ \forall f \in \cF: \abs*{\frac{1}{n} \sum_{i=1}^{n/k} \sum_{j=1}^k \wt{\ell}(f(x_{ij}), \alpha_i) - \cL(f)} \le \eps} \ge 1-\delta
\end{align*}
as long as $n \gtrsim \VC(\cF) \cdot k^3 \log k/ \eps^2$.
\end{proof}

\begin{itemize}
    \item The extra $k$ came from the fact that the values of $\wt{\ell}_B(f) \in [-k, +k]$. Using the fact that w.h.p, for every bag, $\abs{\alpha - p} \le \sqrt{(\log n)/k}$, we can improve the range of $\cF_\cB$ to $[-\sqrt{k \log n}, \sqrt{k \log n}]$ with high probability, translating to a $\VC(\cF) \cdot k^{2} \log k / \eps^2$ sample complexity bound (at the cost of some extra $\log n$ factors).
    \item By comparison, using a Rademacher style analysis, one can get an improved sample complexity of $\VC(\cF) \cdot k \log k /\eps^2 + k^2/\eps^2$. \GLcomment{I believe this is what is done in \cite{busa2023easy}.}
\end{itemize}

\section{Linear Proportion Rule}
Let us consider the following loss function.
\begin{align*}
    \wh{\ell}(f, B) \coloneqq \En f(x) + \En y - 2 \cdot \prn*{ \alpha \cdot \sum_{i=1}^k f(x_i) - (k-1) \En f(x) \En y}
\end{align*}

It can be verified that $\En \wh{\ell}(f, B) = \cL(f)$.


\section{Random Classification Noise Example}
Consider the following example. Suppose $x \sim \mathrm{Unif}(\pm 1)$ and $y = \ind{x \ge 0}$ with probability $p$, $y = \ind{x < 0}$ with probability $1-p$ for some choice of $p \in [0, 1/2]$. Suppose we want to evaluate the loss of the Bayes-optimal classifier $f^\star(x) = \ind{x \ge 0}$. That is, we want to estimate the parameter $p$ given a bag.

The bag $\crl{x_1, x_2, \cdots, x_k, \alpha}$ can be equivalently represented by two values that we observe $n_x$ and $n_y$, where 
\begin{align*}
    n_x \sim \bin(k, 1/2), \quad\text{and} \quad n_y \sim \bin(n_x, 1-p) + \bin(k-n_x, p).
\end{align*}

\begin{problem}
    Given observations $(n_x, n_y)$, compute an unbiased estimator $\wh{p}$ of the loss.
\end{problem}

We already know that the EasyLLP estimator and the Square Loss estimator are unbiased estimators of the loss in general, so they are also unbiased estimators in this special case with random classification noise. Let us verify this explicitly.

\paragraph{Square Loss.}
In this case, the square loss estimator can be written as
\begin{align*}
    \wh{p}_\mathrm{sq} \coloneqq \frac{1}{k} (n_x - n_y)^2.
\end{align*}
Let us compute the expectation conditioned on the value of $n_x$.
\begin{align*}
    \En \brk*{\wh{p}_\mathrm{sq} ~|~ n_x }= \frac{1}{k} \prn*{ n_x^2 - 2n_x \cdot \En\brk{n_y ~|~ n_x} + \En\brk{n_y^2 ~|~ n_x} }.
\end{align*}
Furthermore we can explicitly compute the moments of $n_y$.
\begin{align*}
    \En\brk{n_y ~|~ n_x} &= n_x(1-p) + (k-n_x)p = n_x(1-2p) + kp\\
    \En\brk{n_y^2 ~|~ n_x} &= n_x(1-p)p + n_x^2 (1-p)^2 + (k-n_x)(1-p)p + (k-n_x)^2 p^2 + 2 n_x (k - n_x) (1-p) p \\
    &= k(1-p)p +  n_x^2 (1-p)^2 + (k-n_x)^2 p^2 + 2 n_x (k - n_x) (1-p) p.
\end{align*}
Plugging these values in we get
\begin{align*}
    \En \brk*{\wh{p}_\mathrm{sq} ~|~ n_x } &= \frac{1}{k} \big( n_x^2 - 2n_x \cdot \prn*{n_x(1-2p) + kp} + \\
    &\quad\quad\quad k(1-p)p +  n_x^2 (1-p)^2 + (k-n_x)^2 p^2 + 2n_x (k - n_x) (1-p) p \big) \\
    &= \frac{1}{k} \big( n_x^2 - n_x^2 (2-4p) - 2n_x k p  \\
    &\quad\quad\quad + k(1-p)p + n_x^2 (1-2p+p^2) + k^2p^2 - 2kn_x p^2 + n_x^2 p^2 + 2n_x k(1-p)p+ n_x^2 (2p^2 - 2p) \big).\\
    &= \frac{n_x^2}{k} \big(  1-2+4p + 1 - 2p + p^2 + p^2 + 2p^2 - 2p \big) \\
    &\quad\quad\quad + \frac{n_x}{k} \big( -2kp - 2kp^2 + 2k(1-p)p\big) \\
    &\quad\quad\quad + \frac{1}{k} \big( k(1-p)p + k^2 p^2 \big) \\
    &= \frac{n_x^2}{k} (4p^2) - n_x (4p^2) + (1-p)p + kp^2.
\end{align*}
From here we can take expectation with respect to $n_x$ to get
\begin{align*}
    \En \brk*{\wh{p}_\mathrm{sq} } &= \prn*{\frac{1}{4} + \frac{k}{4}} \prn*{4p^2} - \frac{k}{2} (4p^2) + (1-p)p + kp^2 = p.
\end{align*}

\paragraph{EasyLLP.} Let's check that EasyLLP is unbiased, too. For this setting the EasyLLP estimator becomes
\begin{align*}
    \wh{p}_\mathrm{easy} \coloneqq n_x - \frac{2}{k} n_x n_y + n_y  - \frac{k}{2} + \frac{1}{2}.
\end{align*}
First let us condition on $n_x$ and compute the expected value.
\begin{align*}
    \En \brk*{ \wh{p}_\mathrm{easy} ~|~ n_x } &= n_x - \frac{2}{k} n_x (n_x(1-2p) + kp) + n_x(1-2p) + kp - \frac{k}{2} + \frac{1}{2} \\
    &= \frac{2}{k} n_x^2 (2p-1) + n_x (2 - 4p) + kp - \frac{k}{2} + \frac{1}{2}.
\end{align*}
Now taking expectation with respect to $n_x$ we compute that
\begin{align*}
    \En \brk*{ \wh{p}_\mathrm{easy} } = \prn*{\frac{1}{2} + \frac{k}{2}} (2p-1) + \frac{k}{2} (2-4p) + kp - \frac{k}{2} + \frac{1}{2} = p.
\end{align*}

\begin{proposition}
We can rewrite the estimators for EasyLLP and SquareLoss as follows
\begin{align*}
    \wh{p}_\mathrm{easy} &\coloneqq \prn*{ \frac{n_y - n_x}{k - 2n_x} - \frac{1}{2}} \cdot \frac{1}{k} \prn*{k - 2n_x}^2 + \frac{1}{2}.\\
    \wh{p}_\mathrm{sq} &\coloneqq \prn*{ \frac{n_y - n_x}{k - 2n_x} }^2 \cdot \frac{1}{k} \prn*{k - 2n_x}^2.
\end{align*}
\end{proposition}
Note that the term $\frac{n_y - n_x}{k - 2n_x}$ is the result of moment matching, i.e., if we estimate $p$ by solving the equation
\begin{align*}
    n_y \overset{\mathrm{set}}{=} n_x (1-p) + (k-n_x) p \quad \Rightarrow p\approx \frac{n_y - n_x}{k - 2n_x}.
\end{align*}


\section{Learning Rules}
We consider learning with a loss function $\ell: \bbR \times \bbR \to \bbR_+$.

\subsection{Surrogate Label Approach}
The first and most natural approach is to convert this problem into the standard supervised learning problem. Specifically, we consider using surrogate labels. Given a bag $B$ we can generate the random labeled dataset $(x_1, \wt{y}_1), \cdots, (x_k, \wt{y}_k)$ where the $\wt{y} \sim \mathrm{Ber}(\alpha)$. Given $n$ bags, we then solve the ERM problem
\begin{align*}
    \wh{f} \coloneqq \argmin_{f \in \cF} \frac{1}{nk} \sum_{i=1}^n \sum_{j=1}^k \ell \prn*{ h(x_{ij}), \wt{y}_j }. \numberthis\label{eq:surrogate-loss}
\end{align*}

Other modifications to Eq.~\pref{eq:surrogate-loss} can be found in the EasyLLP paper \cite{busa2023easy}. They study some modifications which reduce the variance. The benefit is that here we can directly minimize the 0-1 loss, while other approaches cannot do so, since they involve minimizing some surrogate loss function.

\subsection{Label Smoothing / Eventified Loss}
If we are working with losses which can take real-valued inputs, then we can try to learn without surrogate labels. This is called \emph{label smoothing}:
\begin{align*}
    \wh{f} \coloneqq \argmin_{f \in \cF} \frac{1}{nk} \sum_{i=1}^n \sum_{j=1}^k \ell \prn*{ h(x_{ij}), \alpha_j }. \numberthis\label{eq:label-smoothing}
\end{align*}
Note the difference with Eq.~\pref{eq:surrogate-loss}! Instead of using surrogate losses, we directly use the real-valued bag proportion in the loss.

\subsection{Bag-Level Loss}
Another approach is to average the labels directly and use a real-valued loss such as log loss or hinge loss.
\begin{align*}
    \wh{f} \coloneqq \argmin_{f \in \cF} \frac{1}{n} \sum_{i=1}^n \ell \prn*{\frac{1}{k} \sum_{j=1}^k h(x_{ij}), \alpha_j }. \numberthis\label{eq:avg-label}
\end{align*}
\GLcomment{Comment from discussion with Lin: this seems to work better than label smoothing, but unsure why. Could be interesting to come up with justification for this?}

\subsection{MLE approach}
The likelihood of the bag can be written as
\begin{align*}
    \ell(f | B) = \sum_{{\bf{y}}\in \crl{0,1}^k: \sum y_i = k \alpha} \prod_{i=1}^k f(x_i)^{y_i} (1-f(x_i))^{1-y_i}.
\end{align*}
Thus we can minimize the loss
\begin{align*}
    \wh{f} \coloneqq \argmin_{f \in \cF} \frac{1}{n} \sum_{i=1}^n \log \ell(f| B_i). \numberthis \label{eq:mle-loss}
\end{align*}
However, this is computationally intractable to minimize, unless the number of bags is small. But note that we can get stochastic gradients for the loss by randomly sampling a $\alpha$-fraction subset and then computing the gradient with respect to the term in the loss given by that choice of $\bf{y}$.

\GLcomment{There is also a poisson approximation. The chat with Lin has the details.}


% \section{Some questions}
% \begin{question} What are the benefits/drawbacks of each approach? Which learning rule should we from a theoretical perspective? 
% \begin{enumerate}
%     \item It seems that the benefit of the surrogate label approach is that one can directly minimize the 0-1 error (at least theoretically), but other approaches can only minimize a convex surrogate.
%     \item How does the bag-level loss compare to the eventified / label smoothing loss? \GLcomment{see jamboard for square loss calculation.}
% \end{enumerate}
% \end{question}

% \begin{question}
% An EM-style approach for the MLE loss where instead of the sum, we take the most plausible labeling given by $f$, and jointly optimize both $f$ as well as the labeling produced by $f$. See, e.g., Barucic and Kybic ``Fast Learning from Label Proportions with Small Bags''. Does this work?
% \end{question}

% \begin{question} Is overfitting to soft labels an issue for the approaches \pref{eq:label-smoothing} and \pref{eq:avg-label}? How can we see this phenomenom? (See EasyLLP paper).
% \begin{enumerate}
%     \item Run experiment where you train same model and loss (1) where the labels are provided and (2) where only the aggregate labels are provided. Does (2) suffer from overfitting when (1) does not? How do we quantify this behavior, or understand why it occurs?
% \end{enumerate}
% \end{question}

% \begin{question} Active learning setting. Suppose we have unlabeled bags $B_1, \cdots, B_n$. How many aggregate labels do we need to query to learn an $\eps$-optimal predictor $\wh{f}$?
% \end{question}



% \section{Transfer Learning with Aggregate Labels}

% We discuss a problem setting where one does transfer learning with aggregate labels. In this setting, we have non-private tasks (where we get the true classification labels) as well as private tasks (where we only have access to aggregate labels). The goal is to do well on the private task. For example, suppose one is training an image classifier using aggregate data. They might want to leverage representations that are learned by training a network on public datasets like MNIST / CIFAR. Since aggregate training data is less helpful, we would like to do as well as we can with few samples from the private task.

% Formally let $\cT = \prn{ \cD_1, \cdots, \cD_T}$ denote the set of $T$ supervised learning tasks over input space $\cX = \bbR^d$ and label space $\cY = \bbR$. For these tasks we have datasets $S_1, \cdots, S_T$ where each dataset $S_t \coloneqq \crl{(x_{ti}, y_{ti})}_{i =1}^n$ is sampled i.i.d.~from $\cD_t$. Also denote $\ell: \cY \times \cY \to \bbR$ to be a loss function. We denote $\cL_{t}(f) \coloneqq \En_{(x,y) \sim \cD_t} \brk*{\ell(f(x), y)}$ as well as $\wh{\cL}_{t}(f) \coloneqq \wh{\En}_{S_t} \brk*{\ell(f(x), y)}$.

% We also denote task $T+1$ as $\cD_{T+1}$ to be a task where we get aggregate training data from. The goal is to minimize the test error on $\cD_{T+1}$, i.e., find some $\wh{f}: \cX \to \cY$ such that
% \begin{align*}
%     \cL_{T+1}(\wh{f}) - \inf_{f \in \cF} \cL_{T+1}(f) \le \eps,
% \end{align*}
% where $\cL_{T+1}(f) \coloneqq \En_{(x,y) \sim \cD_{T+1}} \brk*{ \ell (f(x), y)} \le \epsilon.$

% \subsection{Specific Problem Assumptions} Here is a proposal for a specific problem setup where one can study transfer learning to aggregate label tasks.

% \begin{assumption}[Realizability]
% For each task $t \in [T+1]$, the distribution is realizable w.r.t.~some labeling function that only depends on the first $r$ coordinates: $y = f_t^\star(x_{:r})$.
% \end{assumption}

% \GLcomment{we might need an assumption on task diversity.}

% \subsection{Learning Rule}
% We consider the following learning rule that first learns a good representation using a two-layer NN, and then learns a new head on the aggregate task. Let $\sigma(x) = \mathrm{ReLU}(x)$, $a \in \bbR^m$, $W \in \bbR^{m \times d}$, $b \in \bbR^m$, and $\theta = (a, W, b)$. We denote a neural network as $f_\theta(x) \coloneqq \sum_{i=1}^m a_j \sigma( w_j^\top x + b_j)$. We will train a two-layer NN on the supervised learning tasks:
% \begin{align*}
%     \wh{\theta} = \argmin_{W, b, \crl{a_1, \cdots, a_T}} \frac{1}{T} \sum_{t=1}^T \wh{\cL}_t\prn*{f_{(a_t, W, b)}} + \mathrm{reg.}
% \end{align*}

% Afterwards, we will retrain the head only for the new task:
% \begin{align*}
%     \wh{a}_{T+1} = \argmin_{a} \wh{\cL}^\mathrm{(agg)}_{T+1}\prn*{ f_{(a, \wh{W}, \wh{b})} } + \mathrm{reg}.
% \end{align*}

% Notice that here we depart from the classic transfer learning setup because we will use an aggregate learning algorithm to train the linear head.

% \GLcomment{Another learning rule to consider is to learn the aggregate task simultaneously with the classification tasks. Generally this is not really aligned with transfer learning practice, but maybe in the specific application (with temporal correlations) it can be done.}

% We still need to specify the aggregate learning rule. One possible choice is the EasyLLP one.

% In all experiments, measure the excess risk as a function of the number of training examples for the aggregate task.
% \subsection{Experimental Setup}
% \begin{itemize}
%     \item \textbf{Baseline 1:} train only the aggregate task using the true labels via ERM.
%     \item \textbf{Baseline 2:} train only the aggregate task using EasyLLP.
%     \item \textbf{Baseline 3:} train using standard transfer learning to learn the new classifier.
%     \item \textbf{Experiment 4:} Train using the proposed learning method.
% \end{itemize}
% We would expect the sample complexity to increase from $3\to 4 \to 1 \to 2$.

% Experiment Ideas:
% \begin{itemize}
%     \item Learn sparse parities.
%     \item Learn the hermite polynomials functions from Damian et al.
%     \item Training on MNIST: the classification tasks are learning digits $0-7$ and the aggregate task is $8$ vs $9$, or classification tasks are comparing $0-4$ to $5-9$ and the aggregate task is $0-9$.
% \end{itemize}


